Stochastic Gradient Descent on Nonconvex Functions with General Noise Models

Stochastic Gradient Descent (SGD) is a widely deployed optimization procedure throughout data-driven and simulation-driven disciplines, which has drawn a substantial interest in understanding its global behavior across a broad class of nonconvex problems and noise models. Recent analyses of SGD have made noteworthy progress in this direction, and these analyses have innovated important and insightful new strategies for understanding SGD. However, these analyses often have imposed certain restrictions (e.g., convexity, global Lipschitz continuity, uniform Holder continuity, expected smoothness, etc.) that leave room for innovation. In this work, we address this gap by proving that, for a rather general class of nonconvex functions and noise models, SGD's iterates either diverge to infinity or converge to a stationary point with probability one. By further restricting to globally Holder continuous functions and the expected smoothness noise model, we prove that -- regardless of whether the iterates diverge or remain finite -- the norm of the gradient function evaluated at SGD's iterates converges to zero with probability one and in expectation. As a result of our work, we broaden the scope of nonconvex problems and noise models to which SGD can be applied with rigorous guarantees of its global behavior.

==> sections/analysis_radial_growth.tex <==
Here, we prove \cref{lemma-examples-radial-assumptions} in \cref{subsection-examples-radial}, and \cref{theorem-radial-growth} in \cref{subsection-radial-growth}.

\subsection{Examples of Radial Growth Condition} \label{subsection-examples-radial}

\subsection{Iterate Divergence Occurs with Probability Zero} \label{subsection-radial-growth}

Here, we prove \cref{theorem-radial-growth}. We begin by considering the event on which $\lbrace \norm{\theta_k}_2 \rbrace$ is diverging. Then, on this event, we can define a sequence of stopping times, starting with $\tau_0 = 0$, by
\begin{equation}
\tau_{k} = \min \left\lbrace j > \tau_{k-1} : F(\theta_{j}) > F(\theta_{\tau_{k-1}}) + 1 \right\rbrace.
\end{equation}
On the event of $\lbrace \norm{\theta_k}_2 \rbrace$ diverging, \cref{A5} implies that each of the above stopping times is finite with probability one. Moreover, on the event of the iterates diverging, $\tau_{k} \geq k$ with probability one. 

Now, for all $k+1 \in \mathbb{N}$, let $\mathcal{F}_{\tau_k}$ denote the stopped $\sigma$-algebra corresponding to $\tau_k$.

==> sections/radial_growth.tex <==
We now turn our attention to the case in which the divergence of the iterates is undesirable (i.e., $\inlinePrb{\mathcal{A}_1} = 0$ in \cref{theorem-convergence-local-holder-general-noise}). One would hope that such behavior could fully avoided by requiring coercivity of the objective function, as formalized in the following assumption.

\begin{assumption} \label{A5}
For any sequence $\lbrace \varphi_k : k+1\in \mathbb{N} \rbrace \subset \mathbb{R}^p$ that diverges to infinity (i.e., $\lim_{k \to \infty} \inlinenorm{ \varphi_k }_2 = \infty$), $\liminf_{k \to \infty} F(\varphi_k) = \infty$. 
\end{assumption}

Unfortunately, this does appear to be sufficient to ensure that $\inlinePrb{ \mathcal {A}_1 } = 0$ (i.e., that the iterates of SGD do not diverge). To intuitively understand why this might be the case, consider an objective function $F : \mathbb{R} \to \mathbb{R} $ that is comparable to $\log(\log(|\theta|))$ for all $\theta$ that are sufficiently far from the origin. This comparison implies that such an $F$ satisfies \cref{A5}. 

On the other hand, for sufficiently large $|\theta|$, such a function grows so slowly that it is almost indistinguishable from no growth at all. Furthermore, if, say, $X$ is an fair Rademacher variable and
\begin{equation}
\dot f(\theta,X) = \dot F(\theta) + |\theta| X,
\end{equation}
then the SGD iterates would almost behave as a scaled simple random walk. It then follows that because a simple random walk will travel to distances arbitrarily far from the origin, we may not be able to prevent the SGD iterates from diverging. 

This example intuitively demonstrates the need for ensuring a balance between the behavior of the gradient the the noise model. To formalize this concept, we will need to define, for any $r \geq 0$ and any $\phi \in \mathbb{R}^p$,
\begin{equation}
\sup_{ \varphi : \inlinenorm{ \varphi - \phi}_2 \leq r } \frac{ \norm{ \dot{F}(\varphi) - \dot F(\phi) }_2}{\norm{ \varphi - \phi }_2^\alpha} =: L_r(\phi). 
\end{equation}

Under \cref{A4a}, $L_r(\phi)$ exists and is finite for all $r \geq 0$ and $\phi \in \mathbb{R}^p$. We can now state the assumption. 
\begin{assumption} \label{A6}
Let $G$ be defined as in \cref{A3a}, and $\alpha$ be defined as in \cref{A4a}. There exists constants $b > 0$ and $r > 0$ such that
\begin{equation}
b \leq \liminf_{ \inlinenorm{\phi}_2 \to \infty } \frac{\norm{ \dot F(\phi) }_2^2 }{\bigg[ L_r(\phi) + \Ind{ L_r(\phi) = 0 } \bigg] \bigg[  G(\phi)^{\frac{1+\alpha}{2}} + \Ind{ G(\phi) = 0 } \bigg]}.
\end{equation}
\end{assumption}

\cref{A6} states that the gradient function must grow sufficiently rapidly in order to account for the ``second-order'' information (i.e., the H\"{o}lder constant) and for the noise of the stochastic gradients. 

Importantly, \cref{A5,A6} are not equivalent nor is one somehow subsumed by the other. To show this and scope of these assumptions, we state some simple, one-dimensional, deterministic examples that satisfy both \cref{A5,A6} or that satisfy only one of the two assumptions. The calculations are found in \cref{section-analysis-radial-growth}.

\begin{lemma} \label{lemma-examples-radial-assumptions}
All of the following functions satisfy \cref{A1,A4a} in a region bounded away from zero. Moreover,
\begin{enumerate}[leftmargin=*,itemsep=0em]
\item the following functions satisfy both \cref{A5,A6}: $\exp( |\theta| )$, $|\theta|^q$ for $q > 0$, $\log( 1 + |\theta|)$;
\item the following function satisfies \cref{A5} but not \cref{A6}: $\log( \log( 1 + |\theta| ) )$; and
\item the following fucntion satisfies \cref{A6} but not \cref{A5}: $\exp( - \theta^2)$.
\end{enumerate} 
\end{lemma}


These last two examples demonstrate that \cref{A5,A6} are describing two distinct radial behaviors of objective functions and their derivatives. With both of these additional assumptions, we can effectively prove that the iterates cannot diverge. The proof is supplied in \cref{section-analysis-radial-growth}.

\begin{theorem} \label{theorem-radial-growth}
Let $\lbrace \theta_k \rbrace$ be defined as in \eqref{eqn:iterates} and satisfy \cref{P1,P2,P3,P4}. Suppose \cref{A1,A2,A3a,A4a,A5,A6} hold. Then, the following statements hold with probability one:
\begin{enumerate}[leftmargin=*,itemsep=0em]
\item the limit of $\lbrace \norm{ \theta_k }_2 : k+1 \in \mathbb{N} \rbrace$ exists and is finite;
\item there exists a finite random variable, $F_{\lim}$, such that $\lim_{k \to \infty} F(\theta_k) = F_{\lim}$; and
\item $\lim_{k \to \infty} \inlinenorm{ \dot{F}(\theta_k) }_2 = 0$.
\end{enumerate} 
\end{theorem}

In other words, \cref{theorem-radial-growth} strengthens the conclusions of \cref{theorem-convergence-local-holder-general-noise} by preventing the iterates from diverging under the additional restrictions of \cref{A5,A6,P4}.

